A Multi-Wavelength Study of Low Redshift Clusters of Galaxies I. Comparison of X-ray and Mid-Infrared Selected AGNs

Clusters of galaxies have long been used as laboratories for the study of galaxy evolution, but despite intense, recent interest in feedback between AGNs and their hosts, the impact of environment on these relationships remains poorly constrained. We present results from a study of AGNs and their host galaxies found in low-redshift galaxy clusters. We fit model spectral energy distributions (SEDs) to the combined visible and mid-infrared (MIR) photometry of cluster members and use these model SEDs to determine stellar masses and star-formation rates (SFRs). We identify two populations of AGNs, the first based on their X-ray luminosities (X-ray AGNs) and the second based on the presence of a significant AGN component in their model SEDs (IR AGNs). We find that the two AGN populations are nearly disjoint; only 8 out of 44 AGNs are identified with both techniques. We further find that IR AGNs are hosted by galaxies with similar masses and SFRs but higher specific SFRs (sSFRs) than X-ray AGN hosts. The relationship between AGN accretion and host star-formation in cluster AGN hosts shows no significant difference compared to the relationship between field AGNs and their hosts. The projected radial distributions of both AGN populations are consistent with the distribution of other cluster members. We argue that the apparent dichotomy between X-ray and IR AGNs can be understood as a combination of differing extinction due to cold gas in the host galaxies of the two classes of AGNs and the presence of weak star-formation in X-ray AGN hosts.

==> tab1.tex <==
\begin{deluxetable}{ccccccccccccc}
\tabletypesize{\scriptsize}
\tablewidth{0pc}
%\rotate
\tablecaption{Cluster Sample
\label{tabPhotSumm}}
\tablehead{
\colhead{Cluster} & \colhead{z} & \colhead{$\sigma_{v}$} &
\colhead{$N_{\rm members}$} &
\colhead{IRAC AOR(s)} & \colhead{$\nu L_{\nu,obs}(8\mu m)$ Limit} & 
\colhead{MIPS AOR(s)} & \colhead{$\nu L_{\nu,obs}(24\mu m)$ Limit} \\
\colhead{} & \colhead{} & \colhead{$({\rm km\ s^{-1}})$} & \colhead{} &
\colhead{} & \colhead{$(10^{42}\ {\rm erg\ s^{-1}})$} & \colhead{} & 
\colhead{$(10^{41}\ {\rm erg\ s^{-1}})$} \\
\colhead{} & \colhead{(1)} & \colhead{(2)} & \colhead{(3)} & \colhead{(4)} &
\colhead{(5)} & \colhead{(6)} & \colhead{(7)} }
\startdata
Abell 3128 & 0.0595 & 906 & 83 & 25410816 & $0.54$ & 25411072 & $2.6$ \\
Abell 3125 & 0.0616 & 475 & 25 & 25409792 & $0.58$ & 25410048 & $2.6$ \\
Abell 644  & 0.0701 & 952 & 9 & 25409280 & $1.0$ & --- & --- \\
Abell 2104 & 0.1544 & 1242 & 74 & 25411328 & $1.2$ & 25411584 & $1.9$ \\
Abell 1689 & 0.1867 & 1400 & 160 & 4754176, 14696192, 14696448, 14696704, & $1.3$ & 4770048, 4769792, & $2.8$ \\
 &  &  &  & 14696960, 14697216, 14697472, 25411840 &  & 19042304, 19042048 &  \\
Abell 2163 & 0.2007 & 1381 & 27 & 25412352 & $1.8$ & 25412608 & $3.4$ \\
MS 1008.1-1224  & 0.3068 & 1127 & 68 & 25410304 & $0.81$ & --- & --- \\
AC 114  & 0.3148 & 1388 & 159 & 4756480, 12653824, 25412864 & $1.0$ & 4773888, 4774144, 25413120 & $2.2$ \\
\enddata
\tablecomments{Summary of clusters included in the analysis and the observations
contributing to the MIR mosaic images of each cluster.
The extra line beneath Abell 1689 contains
additional AORs that do not fit on a single line.
(1) Redshifts from \citet{mart07}, determined using the biweight estimator
of \citet{beer90}.
(2) Velocity dispersions of cluster members estimated by \citet{mart09}
using the biweight measure of \citet{beer90}.
(3) Total number of galaxies with both MIR and $R$-band coverage identified as
cluster members by \citet{mart07} or extracted from the literature using
their redshift limits.  (4) Astronomical Observation Request (AOR) numbers
of Spitzer observations used to contruct IRAC mosaics. (5) The minimum
detectable observer-frame $8\mu m$ luminosity in each cluster, derived
from the $3\sigma$ lower limit on measurable flux in a ``typical'' part
of the $8\mu m$ mosaic image.
Due to the variable coverage across the cluster, lower luminosites are
detectable in some cluster members than in others.
(6) AORs used to contruct
the $24\mu m$ mosaics.  (7) $3\sigma$ lower limits on detectable $24\mu m$
luminosities.  These are derived in a similar manner to the IRAC limits in 
column (5) and have the same caveats. }
\end{deluxetable}


==> tab2.tex <==
\begin{deluxetable}{cccccccccccc}
\tabletypesize{\scriptsize}
%\tabletypesize{\footnotesize}
\tablewidth{0pc}
%\rotate
\tablecaption{Cluster Member Photometry
\label{tabPhot}}
\tablehead{
\colhead{Name} & \colhead{RA} & \colhead{Dec} & \colhead{B} &
\colhead{V} & \colhead{R} & \colhead{I} & \colhead{$F_{\nu}(3.6\mu m)$} &
\colhead{$F_{\nu}(4.5\mu m)$\ (mJy)} & \colhead{$F_{\nu}(5.8\mu m)$} &
\colhead{$F_{\nu}(8.0\mu m)$\ (mJy)} & \colhead{$F_{\nu}(24\mu m)$} \\
\colhead{} & \colhead{} & \colhead{} & \colhead{} &
\colhead{} & \colhead{} & \colhead{} & \colhead{(mJy)} &
\colhead{(mJy)} & \colhead{(mJy)} & \colhead{(mJy)} & \colhead{(mJy)} \\
\colhead{(1)} & \colhead{(2)} & \colhead{(3)} & \colhead{(4)} & \colhead{(5)} &
\colhead{(6)} & \colhead{(7)} & \colhead{(8)} & \colhead{(9)} & 
\colhead{(10)} & \colhead{(11)} & \colhead{(12)}}
\startdata
a3128-001 & 03:30:37.7 & -52:32:57 & $17.88\pm0.08$ & $16.81\pm0.06$ & $16.21\pm0.06$ & --- & $ 1.37\pm0.08$ & $ 0.90\pm0.08$ & $ 0.66\pm0.17$ & $< 0.77$ & $< 0.84$ \\
a3125-001 & 03:27:20.2 & -53:28:34 & $17.87\pm0.12$ & $16.89\pm0.09$ & $16.29\pm0.09$ & --- & --- & $ 1.37\pm0.14$ & --- & $ 9.49\pm0.85$ & $ 8.68\pm2.28$ \\
a644-011 & 08:17:39.5 & -07:33:09 & $17.29\pm0.12$ & $16.69\pm0.09$ & $16.20\pm0.09$ & --- & $ 2.61\pm0.21$ & $ 2.55\pm0.24$ & $ 3.62\pm0.48$ & $ 5.15\pm0.62$ & --- \\
a2104-001 & 15:40:07.6 & -03:17:06 & $20.59\pm0.16$ & $19.34\pm0.12$ & $18.62\pm0.12$ & $18.05\pm0.11$ & $ 0.18\pm0.02$ & $ 0.13\pm0.01$ & $< 0.08$ & $< 0.19$ & $< 0.07$ \\
a1689-004 & 13:11:29.5 & -01:20:27 & $17.87\pm0.14$ & $16.48\pm0.10$ & $15.75\pm0.10$ & $15.16\pm0.09$ & $ 2.89\pm0.26$ & $ 2.11\pm0.19$ & $ 1.21\pm0.11$ & $ 0.87\pm0.08$ & $< 0.29$ \\
a2163-001 & 16:15:25.8 & -06:09:26 & $20.70\pm0.19$ & $19.69\pm0.16$ & $18.88\pm0.14$ & --- & $ 0.10\pm0.01$ & $ 0.08\pm0.01$ & $< 0.07$ & $< 0.21$ & $< 0.10$ \\
ms1008-001 & 10:10:34.1 & -12:39:52 & $22.58\pm0.12$ & $21.11\pm0.09$ & $20.10\pm0.08$ & $19.41\pm0.08$ & $ 0.08\pm0.01$ & $ 0.07\pm0.01$ & $ 0.04\pm0.01$ & $< 0.05$ & --- \\
ac114-001 & 22:58:52.3 & -34:46:47 & --- & $22.40\pm0.12$ & $21.73\pm0.10$ & $21.40\pm0.11$ & $ 0.00\pm0.00$ & $ 0.00\pm0.00$ & $< 0.01$ & $< 0.02$ & --- \\
\enddata
\tablecomments{Visible and MIR photometry for a small selection of example
galaxies.  The full table is 
available from the online version of the journal.  (1) The name of
this object, constructed from a shorthand of its parent cluster and the
order in which each object appears in the list of cluster members
extracted from NED.  (2-3) Positions of this object in J2000 coordinates,
as derived from the $R$-band images.  (4-7) Visible photometry for each object,
where detectable, in Vega magnitudes.  Fluxes are measured in the $R$-band
Kron-like aperture.  Objects with no quoted magnitudes
in a given band have either no coverage or no detection in that band.  No
upper limits are quoted.  (5-8) MIR fluxes measured in $R$-band Kron-like
aperture.  Where appropriate, $3\sigma$ upper limits on measured MIR fluxes,
derived from the appropriate uncertainty mosaic, are given.  Galaxies with no
quoted upper limit for a given
band have no coverage in the corresponding image.}
\end{deluxetable}

